Nearest Neighbor Normalization Improves Multimodal Retrieval

Multimodal models leverage large-scale pre-training to achieve strong but still imperfect performance on tasks such as image captioning, visual question answering, and cross-modal retrieval. In this paper, we present a simple and efficient method for correcting errors in trained contrastive image-text retrieval models with no additional training, called Nearest Neighbor Normalization (NNN). We show an improvement on retrieval metrics in both text retrieval and image retrieval for all of the contrastive models that we tested (CLIP, BLIP, ALBEF, SigLIP, BEiT) and for both of the datasets that we used (MS-COCO and Flickr30k). NNN requires a reference database, but does not require any training on this database, and can even increase the retrieval accuracy of a model after finetuning.

==> 01_intro_backup.tex <==
\section{Introduction}
\label{sec:intro}
% Teaser with one histogram (CLIP on COCO) with arrow pointing to outlier image with a bunch of captions matched to it. Includes a schematic of how the method works.
% related work

Contrastive image and text models are a fundamental building block of large-scale multimodal text-to-image or image-to-text retrieval systems~\citep{radford2021learning, jia2021scaling, zhang2022contrastive}. These models compute text and image embeddings separately, and during retrieval, a match score is determined by taking a dot product between embeddings. This makes it possible to encode a text query and quickly find a matching image from a database of precomputed embeddings, or vice-versa. Even though the contrastive paradigm is efficient at scale, contrastive models struggle on tasks requiring fine-grained or compositional understanding \cite{krojer-etal-2022-image, thrush2022winoground, yuksekgonul2023visionlanguage, burapacheep2024colorswap}. While methods exist for improving performance, most approaches either require additional training to adapt models across domains or aggregate information from an external database \cite{zhou2022learning, singha2023ad, iscen2023retrievalenhanced}, or are specialized for individual error categories, such as gender bias \cite{wang2021genderneutral, wang2022fairclip, berg2022prompt}. 

%and lag behind their cross-attention counterparts on retrieval accuracy \cite{li2022blip, singh2022flava}. 

\begin{figure}[t!]
    \centering
    \includegraphics[width=.9\linewidth]{figures/teaser.png}
    \vspace{-3mm}
    \caption{\textbf{Method overview.} \nnd\ applies an additive correction at inference time, using bias scores estimated from a reference database of queries.
    }
    \vspace{-7mm}
    \label{fig:teaser}
\end{figure}

% A variety of post-hoc approaches exist to improve retrieval performance in different settings. Some approaches reduce gender and racial biases by neutralizing their effect on model output \cite{wang2021genderneutral, wang2022fairclip, berg2022prompt}. Other methods adapt contrastive models to new domains by adjusting either prompts or parameters \cite{zhou2022learning, singha2023ad, zhao2023testtime} or learning to aggregate information from an external database to improve retrieval \cite{iscen2023retrievalenhanced}. These approaches typically rely on some degree of training or task-specific considerations.


%Gist of first sentence: Another class of "lighter weight" approaches are task agnostic and applied only at inference time (learning-free).

% More broadly, a variety of inference-time methods address difference in distributions between embeddings learned through pretraining and the utility of embeddings for retrieval.

% where contrastive pretraining objectives (e.g. InfoNCE) typically compute all pairwise similarities in a minibatch, 

% Recent training-free inference-time methods seek to address the following issues. 

% \textbf{1.)} While contrastive pre-training objectives like InfoNCE \cite{radford2021learning} compute all pairwise similarities within a batch of examples, retrieval calculates scores independently for each candidate without considering the overall query distribution, which can lead to poor performance when the retrieval and pre-training distributions differ \cite{zhou2023testtime}. Inference-time methods that address this issue include Distribution Normalization (DN), which computes mean text and image embeddings from a small validation set and subtracts them from each embedding \citet{zhou2023testtime}.

% \textbf{2.)} Large sets of embeddings in high-dimensional space often have the \textit{Hubness} problem \citep{radovanovic2010hubs}, where certain retrieval candidates (``hubs'') emerge as nearest neighbors for many queries in high-dimensional embedding spaces, leading to incorrect matches. Existing approaches for addressing Hubness include QBNorm and DBNorm, which compute normalization constants from large reference banks using softmaxes normalized over the entire bank \cite{bogolin2022cross, wang-etal-2023-balance}. These Hubness methods are computationally expensive, requiring match score calculations for every item in the bank---whereas our approach achieves higher retrieval accuracy using only the \textit{k} nearest embeddings, computed efficiently in sublinear time.

% OLD RECENT DN/HUBNESS TEXT from 6/11
One widespread issue affecting retrieval accuracy is the mismatch between training and inference objectives. While contrastive pre-training objectives like InfoNCE \cite{radford2021learning} compute all pairwise similarities within a batch of examples, retrieval calculates scores independently for each candidate without considering the overall query distribution, which can lead to poor performance when the retrieval and pre-training distributions differ \cite{zhou2023testtime}. 
% the pre-training data distribution and contrastive objective, as opposed to the test distribution and downstream retrieval task, leading to learning embeddings that are suboptimal for retrieval. 
Inference-time methods that address this issue include Distribution Normalization (DN), which computes mean text and image embeddings from a small validation set and subtracts them from each embedding \citet{zhou2023testtime}. Other related methods target the \textit{Hubness} problem \citep{radovanovic2010hubs}, where certain retrieval candidates (``hubs'') emerge as nearest neighbors for many queries in high-dimensional embedding spaces, leading to incorrect matches. Existing approaches for addressing Hubness include QBNorm and DBNorm, which compute normalization constants from large reference banks using softmaxes normalized over the entire bank \cite{bogolin2022cross, wang-etal-2023-balance}. 
These Hubness methods are computationally expensive, requiring match score calculations for every item in the bank---whereas our approach achieves higher retrieval accuracy using only the \textit{k} nearest embeddings, computed efficiently in sublinear time.

%Other approaches do not require additional learning and are applied only at inference time. 
%Test time augmentation (TTA) is one popular approach that found success in image classification, where aggregation over input perturbations improves robustness at inference \citep{shanmugam2021better, kim2020learning, simonyan2015deep, szegedy2014going}. \citet{zhou2023testtime} adapts TTA to retrieval by augmenting and aggregating image embeddings. \citet{zhou2023testtime} also proposes Distribution Normalization (DN), a method which computes mean text and image embeddings from a small validation set and subtracts them from each embedding to correct mismatch between training and inference objectives. Our approach utilizes more fine-grained embedding information by finding a different normalization constant for each individual embedding in the retrieval set.

% quantifying bias \sarah{unclear what bias refers to here, since the only context in which we've brought it up yet is gender and race} for each individual embedding that is being retrieved.

% While DN is motivated by the structure of the infoNCE loss, we strive to solve embedding bias, an empirical challenge we identify in image-text retrieval.

% Second sentence describes broad space of TTA methods - Test time augmentation (TTA) \citet{shanmugam2021better} includes blank and blank, and TODO adapt it to retrieval. TODO also propose DN, a method which BLAH. (we don't need to mention anyhting about benchmarking in the intro, this is a related section). Final sentence of this paragraph should distinguish our method from DN. 

% Domain adapation approaches such as \citet{zhou2022learning} and \citet{singha2023ad} learn prompt prefixes while \citet{zancato2023traintesttime} fine-tunes using an augmented dataset with pseudolabels. However, these approaches are focused on classification and are not easily adaptable to general retrieval tasks. \citet{iscen2023retrievalenhanced}, learns how to aggregate labels from similar texts and images from a database to improve retrieval performance. However, this method requires training an aggregation function.

% On the other hand, \citet{zhou2023testtime} proposes a simple approach involving mean-normalizing embeddings according to a validation set, improving retrieval performance with no additional training. \citet{zhou2023testtime} also adapts the test time augmentation (TTA) approach proposed by \citet{shanmugam2021better} to image-text retrieval, aggregating embeddings across many augmentations of a given image. However, since TTA is orthogonal to both our methodology and the main normalization scheme proposed by \citet{zhou2023testtime}, and because \citet{zhou2023testtime} did not release reproducible code for their version of TTA, we do not benchmark it in this paper.

% Drawing inspiration from these methods, we seek to utilize retrieval to normalize contrastive embedding image-text scoring, improving performance without requiring any training.

% \citet{zhou2023testtime} also utilizes test time augmentation (TTA) inspired by \citet{shanmugam2021better} to further improve performance by averaging embeddings across many augmentations of a given image. However, since TTA is orthogonal to both our methodology and the main normalization scheme proposed by \citet{zhou2023testtime}, and because \citet{zhou2023testtime} did not release reproducible code for their version of TTA, we do not benchmark it in this paper.
%Models can also be adapted to domains they are not trained on by learning to use an external memory bank to retrieve relevant knowledge \citep{iscen2023retrievalenhanced}. \neil {elaborate more here -- what background work should we cite?} - TRISTAN: is this about multimodal retrieval?

We introduce Nearest Neighbor Normalization (\nnd), an efficient task-agnostic method for improving the retrieval accuracy of contrastive image-text models (Figure \ref{fig:teaser}). \nnd\ is training-free and adds minimal inference overhead. The key idea is that \nnd\ corrects for the effects of image and caption embeddings that are assigned disproportionately high or low retrieval scores, by normalizing per-candidate scores using the $k$ closest query embeddings from a reference dataset. %Since \nnd\ only requires the $k$ nearest embeddings, which can be computed efficiently in sublinear time, it is much more efficient than previous approaches.
For example, \nnd\ pushes scores for the image of the surfer in Figure~\ref{fig:matching} (a hub that incorrectly matches with large number of query captions in a COCO retrieval task) closer to other image scores, thus improving overall accuracy. %by reducing the influence of a hub.
%\nnd\ corrects key-query matching scores by subtracting \textit{bias} of models toward a retrieved key, which we parameterize as the mean match score between the key and a set of nearest neighbor query vectors in an associated embedding space. 
% Some image or caption embeddings are assigned an unrealistically high score, regardless of the embedding that they are are dotted with. For example, the image of the surfer in Figure \ref{fig:matching} is an image in a retrieval database with high match scores with a disproportionately high number of text queries. In this case, \nnd\ makes the scores for this image smaller, so that they are closer to the scores obtained for other images. %Alternatively, an embedding could generally score very low, in which case our approach would correct for this as well. 
Section \ref{sec:method} provides more details on our approach, and Section \ref{sec:experiments} empirically validates the effect of \nnd\ for a range of models and datasets.

Overall, we contribute a new and conceptually simple approach for improving contrastive retrieval with little compute overhead. In addition to improving retrieval scores consistently for every model and dataset that we tested, \nnd\ outperforms DN, QBNorm, and DBNorm. Our approach is also able to reduce harmful biases such as gender bias. 

% be used to do targeted normalization, such as gender debiasing. 
%we already abbreviate DN on line 61, is it necessary to do it again here? could say "other test-time methods like DN," 
%ok good point - Tristan

%We find that \nnd\ consistently improves model performance on both image and text retrieval for multiple datasets, decreases variance in the distribution of captions matched to images, and reduces unwanted correlations such as gender bias in image retrieval. 

% We introduce Nearest Neighbor Debiasing (\nnd), a training-free scheme for improving the retrieval accuracy of dual encoder models (Figure \ref{fig:teaser}). The intuition behind \nnd\ is simple: the distribution of key-query matching scores does not reflect the ground-truth distribution, %TODO is "ground-truth distribution" best? 
%some retrieved keys (\eg\ the image of the surfer in Figure \ref{fig:matching}) are associated with a disproportionately high (or low) number of queries.
%\nnd\ corrects key-query matching scores by subtracting \textit{bias} of models toward a retrieved key, which we parameterize as the mean match score between the key and a set of nearest neighbor query vectors in an associated embedding space. Section \ref{sec:method} provides more details on our approach, and Section \ref{sec:experiments} empirically validates the effect of \nnd\ on multimodal retrieval for a range of encoder models and query embedding spaces. TODO: what to call "query embedding spaces" 

%In cases where an in-distribution set of alternate queries is used \sumedh{need to explain this here? or can we just point to section 2}, \nnd\ improves performance on both image retrieval and text retrieval for both base and finetuned models, although base models see a greater benefit. \sarah{I think this first statement of results can be more impressive}. Furthermore, we show that \nnd\ quantitatively reduces the kurtosis of the distribution of the number of queries matched with each key, thus having the desirable property of removing outlier keys that are matched with a substantial fraction of queries. 
%Though TODO limitation (it doesn't solve everything), we suggest that \nnd\ is widely useful for cases where TODO. 
%It is extremely compute efficient, and is compatible with black-box embedding models (\eg\ accessible via an API endpoint, without finetuning).
